MASS: MoErging through Adaptive Subspace Selection

Model merging has recently emerged as a lightweight alternative to ensembling, combining multiple fine-tuned models into a single set of parameters with no additional training overhead. Yet, existing merging methods fall short of matching the full accuracy of separately fine-tuned endpoints. We present MASS (MoErging through Adaptive Subspace Selection), a new approach that closes this gap by unifying multiple fine-tuned models while retaining near state-of-the-art performance across tasks. Building on the low-rank decomposition of per-task updates, MASS stores only the most salient singular components for each task and merges them into a shared model. At inference time, a non-parametric, data-free router identifies which subspace (or combination thereof) best explains an input's intermediate features and activates the corresponding task-specific block. This procedure is fully training-free and introduces only a two-pass inference overhead plus a ~2 storage factor compared to a single pretrained model, irrespective of the number of tasks. We evaluate MASS on CLIP-based image classification using ViT-B-16, ViT-B-32 and ViT-L-14 for benchmarks of 8, 14 and 20 tasks respectively, establishing a new state-of-the-art. Most notably, MASS recovers up to ~98% of the average accuracy of individual fine-tuned models, making it a practical alternative to ensembling at a fraction of the storage cost.

==> _vision_table.tex <==
\renewcommand{\arraystretch}{1.5} 
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccccccccccccccccccc@{}}
\toprule
\multicolumn{2}{c}{} &  & \multicolumn{8}{c}{ViT-B/32} &  &  & \multicolumn{8}{c}{ViT-L/14} \\ \cmidrule(lr){4-11} \cmidrule(l){14-21} 
\multicolumn{2}{c}{} &  & \multicolumn{2}{c}{8 tasks} &  & \multicolumn{2}{c}{14 tasks} &  & \multicolumn{2}{c}{20 tasks} &  &  & \multicolumn{2}{c}{8 tasks} &  & \multicolumn{2}{c}{14 tasks} &  & \multicolumn{2}{c}{20 tasks} \\ \cmidrule(lr){4-5} \cmidrule(lr){7-8} \cmidrule(lr){10-11} \cmidrule(lr){14-15} \cmidrule(lr){17-18} \cmidrule(l){20-21} 
\multicolumn{2}{c}{\multirow{-3}{*}{Method}} &  & Acc.(\%) $\uparrow$ & Bits$\downarrow$ &  & Acc.(\%) $\uparrow$ & Bits$\downarrow$ &  & Acc.(\%) $\uparrow$ & Bits$\downarrow$ &  &  & Acc.(\%) $\uparrow$ & Bits$\downarrow$ &  & Acc.(\%) $\uparrow$ & Bits$\downarrow$ &  & Acc.(\%) $\uparrow$ & Bits$\downarrow$ \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF} & Zeroshot &  & 48.4 & {\color[HTML]{656565} 3.6} &  & 57.3 & {\color[HTML]{656565} 3.6} &  & 56.1 & {\color[HTML]{656565} 3.6} &  &  & 64.4 & {\color[HTML]{656565} 11.0} &  & 68.0 & {\color[HTML]{656565} 11.0} &  & 65.1 & {\color[HTML]{656565} 11.0} \\

\cellcolor[HTML]{FFFFFF} & Weight averaging &  & \foo{66.5}{72.3} & {\color[HTML]{656565} 3.6} &  & \foo{64.4}{71.2} & {\color[HTML]{656565} 3.6} &  & \foo{61.1}{67.5} & {\color[HTML]{656565} 3.6} &  &  & \foo{79.4}{83.0} & {\color[HTML]{656565} 11.0} &  & \foo{76.6}{81.0} & {\color[HTML]{656565} 11.0} &  & \foo{71.5}{75.5} & {\color[HTML]{656565} 11.0} \\

\cellcolor[HTML]{FFFFFF} & Task arithmetic &  & \foo{70.8}{76.5} & {\color[HTML]{656565} 3.6} &  & \foo{65.4}{72.2} & {\color[HTML]{656565} 3.6} &  & \foo{60.6}{66.8} & {\color[HTML]{656565} 3.6} &  &  & \foo{84.8}{88.5} & {\color[HTML]{656565} 11.0} &  & \foo{79.3}{83.8} & {\color[HTML]{656565} 11.0} &  & \foo{74.0}{78.0} & {\color[HTML]{656565} 11.0} \\
\cellcolor[HTML]{FFFFFF} & TIES &  & \textbf{\foo{75.1}{81.0}} & {\color[HTML]{656565} 3.6} &  & \foo{68.0}{74.8} & {\color[HTML]{656565} 3.6} &  & \foo{63.4}{69.9} & {\color[HTML]{656565} 3.6} &  &  & \textbf{\foo{86.9}{90.7}} & {\color[HTML]{656565} 11.0} &  & \foo{79.5}{84.1} & {\color[HTML]{656565} 11.0} &  & \foo{75.7}{79.8} & {\color[HTML]{656565} 11.0} \\

\cellcolor[HTML]{FFFFFF} & \textbf{Consensus TA [ours]} &  & \foo{75.0}{80.8} & {\color[HTML]{656565} 3.6} &  & \textbf{\foo{70.4}{77.4}} & {\color[HTML]{656565} 3.6} &  & \textbf{\foo{65.4}{72.0}} & {\color[HTML]{656565} 3.6} &  &  & \foo{86.2}{89.9} & {\color[HTML]{656565} 11.0} &  & \textbf{\foo{82.2}{86.9}} & {\color[HTML]{656565} 11.0} &  & \textbf{\foo{78.9}{83.2}} & {\color[HTML]{656565} 11.0} \\

\multirow{-6}{*}{\cellcolor[HTML]{FFFFFF}\rotatebox[origin=c]{90}{Merging}} & \textbf{Consensus TIES [ours]} &  & \foo{74.8}{80.6} & {\color[HTML]{656565} 3.6} &  & \foo{67.7}{74.5} & {\color[HTML]{656565} 3.6} &  & \foo{63.2}{69.6} & {\color[HTML]{656565} 3.6} &  &  & \textbf{\foo{86.9}{90.7}} & {\color[HTML]{656565} 11.0} &  & \foo{81.5}{86.1} & {\color[HTML]{656565} 11.0} &  & \foo{76.8}{80.9} & {\color[HTML]{656565} 11.0} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } & \cellcolor[HTML]{EFEFEF}{\color[HTML]{333333} Fine-tuned} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}92.8 & {\color[HTML]{656565} 23.3} &  & 90.9 & {\color[HTML]{656565} 40.2} &  & 91.3 & {\color[HTML]{656565} 57.0} &  &  & 95.8 & {\color[HTML]{656565} 79.1} &  & 94.3 & {\color[HTML]{656565} 137.4} &  & 94.7 & {\color[HTML]{656565} 195.8} \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } & Magnitude Pruning &  & \foo{91.3}{98.4} & {\color[HTML]{656565} \textgreater7.1} &  & \foo{85.3}{93.7} & {\color[HTML]{656565} \textgreater7.7} &  & \foo{83.4}{91.2} & {\color[HTML]{656565} \textgreater8.2} &  &  & \foo{95.4}{99.6} & {\color[HTML]{656565} \textgreater23.1} &  & \foo{91.8}{97.2} & {\color[HTML]{656565} \textgreater24.9} &  & \foo{91.2}{96.1} & {\color[HTML]{656565} \textgreater26.8} \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } & Magnitude Masking &  & \foo{86.8}{93.3} & {\color[HTML]{656565} 7.1} &  & \foo{80.7}{88.4} & {\color[HTML]{656565} 7.7} &  & \foo{75.3}{82.1} & {\color[HTML]{656565} 8.2} &  &  & \foo{94.6}{98.7} & {\color[HTML]{656565} 23.1} &  & \foo{91.6}{97.0} & {\color[HTML]{656565} 24.9} &  & \foo{91.6}{96.5} & {\color[HTML]{656565} 26.8} \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } & \textbf{TALL Mask + TA [ours]} &  & \foo{92.6}{99.7} & {\color[HTML]{656565} 7.1} &  & \foo{90.1}{99.1} & {\color[HTML]{656565} 7.7} &  & \foo{90.6}{99.2} & {\color[HTML]{656565} 8.2} &  &  & \foo{95.7}{99.9} & {\color[HTML]{656565} 23.1} &  & \foo{93.1}{98.8} & {\color[HTML]{656565} 24.9} &  & \foo{93.7}{98.9} & {\color[HTML]{656565} 26.8} \\
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \rotatebox[origin=c]{90}{Compression}}} & \textbf{TALL Mask + TIES [ours]} &  & \textbf{\foo{93.0}{100.3}} & {\color[HTML]{656565} 7.1} &  & \textbf{\foo{90.9}{100.0}} & {\color[HTML]{656565} 7.7} &  & \textbf{\foo{91.1}{99.7}} & {\color[HTML]{656565} 8.2} &  &  & \textbf{\foo{95.9}{100.1}} & {\color[HTML]{656565} 23.1} &  & \textbf{\foo{93.4}{99.0}} & {\color[HTML]{656565} 24.9} &  & \textbf{\foo{93.9}{99.1}} & {\color[HTML]{656565} 26.8} \\ \bottomrule
\end{tabular}
}
